TACCL: Guiding Collective Algorithm Synthesis using Communication Sketches

Machine learning models are increasingly being trained across multiple GPUs and servers. In this setting, data is transferred between GPUs using communication collectives such as AlltoAll and AllReduce, which can become a significant bottleneck in training large models. Thus, it is important to use efficient algorithms for collective communication. We develop TACCL, a tool that enables algorithm designers to guide a synthesizer into automatically generating algorithms for a given hardware configuration and communication collective. TACCL uses a novel communication sketch abstraction to get crucial information from the designer to significantly reduce the search space and guide the synthesizer towards better algorithms. TACCL also uses a novel encoding of the problem that allows it to scale beyond single-node topologies. We use TACCL to synthesize algorithms for three collectives and two hardware topologies: DGX-2 and NDv2. We demonstrate that the algorithms synthesized by TACCL outperform the Nvidia Collective Communication Library (NCCL) by up to 6.7x. We also show that TACCL can speed up end-to-end training of Transformer-XL and BERT models by 11%--2.3x for different batch sizes.

==> tex/discussion.tex <==
\camera{\section{Limitations and Future Work}}
\label{discuss}
\sysname uses user-provided communication sketches to guide synthesis of collective algorithms.
Using a three-step technique of relaxed routing, heuristic ordering, and contiguity and exact scheduling,
\sysname generates efficient collectives for multi-node topologies.
We note that \sysname's synthesis technique is not optimal, but has still been proven to synthesize
efficient algorithms when used hand-in-hand with communication sketches.
We also briefly discuss some other aspects of \sysname below:

\myparab{Scalability.} \sysname can synthesize algorithms for large-scale nodes -
we have been able to synthesize an \allgather algorithm for 8 Azure \ndvtwo nodes
using \sysname in under 5 minutes. As compared to NCCL, this algorithm has up-to $1.7\times$
higher algorithm bandwidth for different data sizes. We also evaluated \sysname's synthesis for
8 NVIDIA \dgxtwo nodes (128 GPUs) and found a solution in around 11 hours.
While \sysname scales to multi-node topologies, the synthesis technique
is still based on solving an NP-hard problem that grows exponentially with a quadratic power
with scale. As future work, we would like to scale \sysname further by hierarchically composing
synthesized algorithms.

\myparab{Generality across different topologies.} Apart from hierarchical topologies like
NVIDIA \dgxtwo and Azure \ndvtwo, \sysname can also be applied to non-hierarchical topologies
like a 2D-Torus. We were able to synthesize an \allgather algorithm for a 2D 6x8 Torus using
\sysname. We made use of the symmetry attribute in communication sketches to explore synthesis
for this topology.
However, the amount of exploration we can do with different communication sketches may be
more limited in these cases than for hierarchical topologies.

\myparab{Exploring communication sketches.} Communication sketches have proven effective in
narrowing the search space of algorithms, but more interestingly,
we found that different communication sketches can optimize different ranges of
input sizes. Communication sketches reflect the intuition of the developers, and by intelligently
exploring the space of communication-sketches we could obtain a range of collective algorithms with
different performance characteristics.
Learning an automated controller for communication sketches might an interesting
direction for collective algorithm synthesis in the future.
